Self-training Improves Pre-training for Natural Language Understanding

Unsupervised pre-training has led to much recent progress in natural language understanding. In this paper, we study self-training as another way to leverage unlabeled data through semi-supervised learning. To obtain additional data for a specific task, we introduce SentAugment, a data augmentation method which computes task-specific query embeddings from labeled data to retrieve sentences from a bank of billions of unlabeled sentences crawled from the web. Unlike previous semi-supervised methods, our approach does not require in-domain unlabeled data and is therefore more generally applicable. Experiments show that self-training is complementary to strong RoBERTa baselines on a variety of tasks. Our augmentation approach leads to scalable and effective self-training with improvements of up to 2.6% on standard text classification benchmarks. Finally, we also show strong gains on knowledge-distillation and few-shot learning.

==> SentAugment - NAACL (1)/content/tables.tex <==



\newcommand{\insertapproach}{
\begin{figure*}[t]
	\begin{center}
          %\includegraphics[width=\linewidth]{content/xlmroberta_transfer_dilution.pdf}
        \includegraphics[width=\linewidth]{content/sentaugment}
        \caption{\textbf{The SentAugment approach.} The self-training procedure follows multiple steps; \textbf{Step 1}: A RoBERTa-Large model - the teacher - is finetuned on a downstream task using a cross-entropy loss, \textbf{Step 2}: Task-specific unannotated data is extracted from a large bank of sentences; This step uses task-specific query embeddings (produced by a paraphrastic sentence encoder) to select nearest neighbors from the bank. \textbf{Step 3}: This data is synthetically annotated using the teacher model; top K samples from each class are selected to form the final synthetic dataset; \textbf{Step 4}: A RoBERTa-Large model - the student - is finetuned on this dataset using KL-divergence. Our approach differs from previous work at Step 2, which we show is crucial for open-domain self-training.
            \label{fig:sentaugment}}
        \vspace{-0.2cm}
	\end{center}
\end{figure*}
}


% Results on self-training
\newcommand{\insertselftrain}{
    \begin{table*}[h!]
        \begin{center}
            % \scriptsize
            \resizebox{0.8\linewidth}{!}{
            \begin{tabular}[b]{lccccccccc}
            \toprule
                {\bf Model} & {\bf SST-2} & {\bf SST-5} & {\bf CR} & {\bf IMP} & {\bf TREC} & {\bf NER} & {\bf Avg} \\
                \midrule
                \midrule
                % \multicolumn{3}{l}{Num samples} & 67k & 8.5k & 2.5k & 3.9k & 5k & 12k \\
                % \midrule
                % \midrule
                RoBERTa$_{\text{Large}}$ & 96.5 & 57.8 & 94.8 & 84.6 & \bf 97.8  & 92.7 & 87.4 \\
                RoBERTa$_{\text{Large}}$ + ICP & 93.9 & 55.1 & 93.7 & 84.4 & 97.8  & 92.1 & 86.2 \\
                RoBERTa$_{\text{Large}}$ + ST & \bf 96.7 & \bf 60.4 & \bf 95.7 & \bf 87.7 & \bf 97.8  & \bf 93.3 & \bf 88.6 \\
                \bottomrule
            \end{tabular}
            }
            \caption{Results of self-training on natural language understanding benchmarks. We report a strong RoBERTa-Large baseline, as well as in-domain continued pretraining of this model (ICP) and our self-training approach (ST).
            \label{tab:selftrain}}
        \end{center}
       \vspace{-0.4cm}
    \end{table*}
}


% Few-shot learning
\newcommand{\insertfewshot}{
    \begin{table*}[h]
        \begin{center}
            % \scriptsize
            \resizebox{\linewidth}{!}{
            \begin{tabular}[t]{lccccccc}
            \toprule
                {\bf Model} &  {\bf SST-2} & {\bf SST-5} & {\bf CR} & {\bf IMP} & {\bf TREC} & {\bf NER} & {\bf Avg} \\
                % \midrule
                % \midrule
                % Num samples & 67k & 8.5k & 2.5k & 3.9k & 5k & 12k \\
                % \midrule
                % \midrule
                % RoBERTa-Large & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0  \\
                % RoBERTa-Large + ST & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
                \midrule
                \midrule
                \multicolumn{1}{l}{Num samples} & 40 & 100 & 40 & 40 & 120 & 200 & - \\
                \midrule
                \midrule
                RoBERTa$_{\text{Large}}$ & 83.6$\pm$2.7 & 42.3$\pm$1.6 & 88.9$\pm$1.7 & 77.3$\pm$2.8 & 90.9$\pm$2.5 & 49.0$\pm$1.7 & 72.0$\pm$2.2\\
                RoBERTa$_{\text{Large}}$ + ST & \textbf{86.7$\pm$2.3} & \textbf{44.4$\pm$1.0} & \textbf{89.7$\pm$2.0} & \textbf{81.9$\pm$1.4} & \textbf{92.1$\pm$2.4} & \textbf{58.4$\pm$1.4} & \textbf{75.5$\pm$1.8} \\
                \bottomrule
            \end{tabular}
            }
            \caption{Results of self-training for few-shot learning, using only 20 samples per class.
            \label{tab:fewshot}}
        \end{center}
       \vspace{-0.4cm}
    \end{table*}
}




% Results on knowledge-distillation
\newcommand{\insertkd}{
    \begin{table*}[h!]
        \begin{center}
            % \scriptsize
            \resizebox{0.85\linewidth}{!}{
            \begin{tabular}[t]{lccccccc}
            \toprule
                {\bf Model} & {\bf KD-data} & {\bf SST-2} & {\bf SST-5} & {\bf CR} & {\bf IMP} & {\bf TREC} & {\bf Avg} \\
                \midrule
                \midrule
                \multicolumn{8}{l}{\it Models trained directly on the training set of each downstream task} \\
                \midrule
                \midrule
                RoBERTa$_{\text{Large}}$ & - & \bf 96.5 & \bf  57.8 & \bf 94.8 & \bf 84.6 & \bf 97.8 & \bf 86.3 \\
                RoBERTa$_{\text{Small}}$ & - & 92.0 & 49.0 & 88.7 & 83.8 & 96.4 & 82.0 \\
                \midrule
                \midrule
                \multicolumn{8}{l}{\it Models distilled using the same number of sentences as in the train set (cf. Table~\ref{tab:datasets})} \\
                \midrule
                \midrule
                RoBERTa$_{\text{Small(Large)}}$ & GT & 92.4& 49.7 & 89.6 & 84.4 & 96.6 & 82.5 \\
                RoBERTa$_{\text{Small(Large)}}$ & RD & 90.7 & 47.5 & 87.4 & 69.1 & 90.8 & 77.1 \\
                RoBERTa$_{\text{Small(Large)}}$ & SA & 91.8 & 50.7 & 88.2 & 84.6 & 94.4 & 81.9 \\
                \midrule
                \midrule
                \multicolumn{8}{l}{\it Models distilled using more unsupervised sentences (100k sentences)} \\
                \midrule
                \midrule
                RoBERTa$_{\text{Small(Large)}}$ & RD & 92.5 & 51.2 & 92.4 & 78.1 & 96.2 & 82.1 \\
                RoBERTa$_{\text{Small(Large)}}$ & SA & \bf 94.2 & \bf 57.6 & \bf 92.6 & \bf 85.5 & \bf 97.0 & \bf 85.4 \\
                % %\midrule
                % \midrule
                % \midrule
                % \multicolumn{6}{l}{Models distilled from RoBERTa-Large}\\
                % \midrule
                % \midrule
                % RoBERTa$_{\text{Small}}$ & ground-truth & 00.0 & 00.0 & 00.0 & 00.0 \\
                % RoBERTa$_{\text{Small}}$ & random-100k & 00.0 & 00.0 & 00.0 & 00.0 \\
                % RoBERTa$_{\text{Small}}$ & filtered-100k & 00.0 & 00.0 & 00.0 & 00.0 \\
                \bottomrule
            \end{tabular}
            }
            \caption{Results of knowledge-distillation using ground-truth (GT), random (RD), or data-selected data (SA) as unnanotated sentences. We distill a RoBERTa-Large model of 24 layers into a RoBERTa-Small model with $100\times$ less parameters. \label{tab:kd}}
        \end{center}
       \vspace{-0.4cm}
    \end{table*}
}


% Ablation study - GT vs RD vs SA
\newcommand{\insertgroundtruth}{
    \begin{table*}[h!]
        \begin{center}
            % \scriptsize
            \resizebox{0.8\linewidth}{!}{
            \begin{tabular}[b]{lccccccc}
            \toprule
                {\bf Model} & {\bf KD-data} & {\bf SST-2} & {\bf SST-5} & {\bf CR} & {\bf IMP} & {\bf TREC} & {\bf Avg} \\
                \midrule
                \midrule
                RoBERTa$_{\text{Small(Large)}}$ & GT & 92.4& 49.7 & 89.6 & 84.4 & 96.6 & 82.5 \\
                RoBERTa$_{\text{Small(Large)}}$ & RD & 90.7 & 47.5 & 87.4 & 69.1 & 90.8 & 77.1 \\
                RoBERTa$_{\text{Small(Large)}}$ & DA & 91.8 & 50.7 & 88.2 & 84.6 & 94.4 & 81.9 \\
                \bottomrule
            \end{tabular}
            }
            \caption{Results of knowledge-distillation using ground-truth (GT), random (RD), or data-selected data (DA) as unnanotated sentences. We distill a RoBERTa-Large model of 24 layers into a RoBERTa-Small model with 100\* less parameters. \jingfei{TODO: rerun to validate all numbers} \label{tab:kd}}
        \end{center}
       \vspace{-0.4cm}
    \end{table*}
}



% Ablation study - impact of data augmentation technique
\newcommand{\insertaugmentation}{
    \begin{table}[h!]
        \begin{center}
            % \scriptsize
            \resizebox{1\linewidth}{!}{
            \begin{tabular}[h!]{llccccc}
            \toprule
                {\bf Model} & {\bf Selection} & {\bf $\mathcal{C}$} & {\bf SST-5} & {\bf CR} & {\bf NER} & {\bf Avg} \\
                \midrule
                % \midrule
                % \multicolumn{2}{l}{Num samples} & 8.5k & 2.5k & 3.9k & 7.5k & 5.5k  \\
                % \midrule
                % \midrule
                RoBERTa$_{\text{Large}}$ + ST & all-avg & $\mathcal{O}(Md^2)$ & 60.0 & 94.7 & 92.8 & 82.5 \\
                RoBERTa$_{\text{Large}}$ + ST & label-avg & $\mathcal{O}(KMd^2)$ & \bf 60.4 & \bf 95.7 & 93.1 & \bf 83.1 \\
                RoBERTa$_{\text{Large}}$ + ST & per-sent & $\mathcal{O}(NMd^2)$ & 60.1 & 95.4 & \bf 93.3 & 82.9 \\
                \bottomrule
            \end{tabular}
            }
            \caption{Impact of data augmentation technique. $\mathcal{C}$ is the complexity, $M$ the size of the bank of sentences, $K$ the number of labels (or clusters), $N$ the size of the downstream training set and $d$ the embedding size.\label{tab:augmentation}}
        \end{center}
       \vspace{-0.4cm}
    \end{table}
}

% Ablation study - impact of sentence embeddings
\newcommand{\insertembedding}{
    \begin{table}[h!]
        \begin{center}
            % \scriptsize
            \resizebox{1\linewidth}{!}{
            \begin{tabular}[b]{lcccccc}
            \toprule
                {\bf Model} & {\bf Embedding} & {\bf dim} & {\bf SST-5} & {\bf CR} & {\bf NER} & {\bf Avg} \\
                \midrule
                % \midrule
                % \multicolumn{2}{l}{Num samples} & 8.5k & 2.5k & 3.9k & 7.5k & 5.5k  \\
                % \midrule
                % \midrule
                RoBERTa$_{\text{Large}}$ + ST & avg-w2v & 300 & 59.4 & 95.2 & 92.9 & 82.5 \\
                RoBERTa$_{\text{Large}}$ + ST & uSIF & 300 & 59.9 & 95.0 & 93.1 & 82.7 \\
                RoBERTa$_{\text{Large}}$ + ST & SASE & 256 & \bf 60.4 & \bf 95.7 & \bf 93.1 & \bf 83.1 \\
                \bottomrule
            \end{tabular}
            }
            \caption{Impact of sentence embedding method: average-word2vec, uSIF with ParaNMT and SASE. \label{tab:embeddings}}
        \end{center}
       \vspace{-0.4cm}
    \end{table}
}



% Ablation study - impact of size of external corpus
\newcommand{\insertmemory}{
    \begin{table}[h!]
        \begin{center}
            % \scriptsize
            \resizebox{1\linewidth}{!}{
            \begin{tabular}[b]{lcccccc}
            \toprule
                {\bf Model} & {\bf \#lines} & {\bf \#words} & {\bf SST-5} & {\bf CR} & {\bf NER} & {\bf Avg}  \\
                \midrule
                % \midrule
                % \multicolumn{2}{l}{Num samples} & 8.5k & 2.5k & 3.9k & 7.5k & 5.5k  \\
                % \midrule
                % \midrule
                RoBERTa$_{\text{Large}}$ + ST & 50m & 1B & 59.5 & 95.4 & 92.8 & 82.6  \\
                RoBERTa$_{\text{Large}}$ + ST & 250m & 5B & 59.5 & \bf 95.7 & 92.9 & 82.7  \\
                RoBERTa$_{\text{Large}}$ + ST & 1B & 20B & \bf 60.4 & \bf 95.7 & \bf 93.1 & \bf 83.1  \\
                RoBERTa$_{\text{Large}}$ + ST & 5B & 100B & 60.0 & 95.3 & \bf 93.1 & 82.8  \\
                \bottomrule
            \end{tabular}
            }
            \caption{Impact of sentence bank size (number of lines and words) on self-training results. \label{tab:memory}}
        \end{center}
       \vspace{-0.4cm}
    \end{table}
}

% Datasets
\newcommand{\insertdatasets}{
    \begin{table*}[t]
        \begin{center}
            % \scriptsize
            \resizebox{0.9\linewidth}{!}{
            \begin{tabular}[b]{lllrc}
            \toprule
                {\bf Dataset} & {\bf task} & {\bf domain} & {\bf \#train} & {\bf \#classes}\\
                \midrule
                % \midrule
                % \multicolumn{2}{l}{Num samples} & 8.5k & 2.5k & 3.9k & 7.5k & 5.5k  \\
                % \midrule
                % \midrule
                SST-2 & sentiment analysis & movie reviews & 67349 & 2 \\
                SST-5 & sentiment analysis & movie reviews & 8544 & 5\\
                CR & product classification & product reviews & 2500 & 2  \\
                IMP & hate-speech classification & forum conversations & 3947 & 2 \\
                TREC & question-type classification & short questions & 5001 & 6 \\
                CoNLL & named entity recognition & news stories & 11663 & 5  \\

                \bottomrule
            \end{tabular}
            }
            \caption{Downstream tasks used for evaluation. \label{tab:datasets}}
        \end{center}
       \vspace{-0.4cm}
    \end{table*}
}

% Ablation study - impact of soft label vs. discrete label
\newcommand{\insertlabel}{
    \begin{table}[h!]
        \begin{center}
            % \scriptsize
            \resizebox{1\linewidth}{!}{
            \begin{tabular}[b]{lccccc}
            \toprule
                {\bf Model} & {\bf label type} & {\bf SST-5} & {\bf CR} & {\bf NER} & {\bf Avg} \\
                \midrule
                % \midrule
                % \multicolumn{2}{l}{Num samples} & 8.5k & 2.5k & 3.9k & 7.5k & 5.5k  \\
                % \midrule
                % \midrule
                RoBERTa$_{\text{Large}}$ + ST & discrete & 59.1 & 94.7 & 92.8  & 82.2  \\
                RoBERTa$_{\text{Large}}$ + ST & logits &  \bf 60.4 & \bf 95.7 & \bf 93.1  & \bf 83.1 \\
                \bottomrule
            \end{tabular}
            }
            \caption{Impact of label type on self-training results. \label{tab:logits}}
        \end{center}
       \vspace{-0.4cm}
    \end{table}
}



%%% Retrieval examples
\newcommand{\insertexamples}{
    \begin{table*}[h]
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{l}
        \toprule
        \bf Movie reviews - Retrieved sentences for the \textit{positive} class of the SST-5 task\\
        \midrule
        Great film with a timeless story and spectacular acting. \\
        An amazing film that is fast-paced, entertaining, funny and horrific in equal measure. \\
        Overall this movie is very funny, charming, full of wit and depth with excellent acting and a perfect script. \\
        \midrule
        \bf Movie reviews - Retrieved sentences for the \textit{negative} class of the SST-5 task\\
        \midrule
        This is bland, uninspired, humorless filmmaking at its worst. \\
        It is a slow and stodgy drama, bogged down by clumsy writing and outrageously bad performances. \\
        This movie was terribly boring, but so forgettable as well that it didn't stand out for how awful it was.. \\
        \midrule
        \bf Toxic comments - Retrieved sentences for the \textit{hateful} class of the IMP task \\
        \midrule
        Lol you people are fucking retarded. \\
        fuzzy you are such a dumb fucking piece of shit just shut your god damn mouth. \\
        As many as it takes to shame you into realizing you're a gullible moron. \\
        \midrule
        \bf Product reviews - Retrieved sentences for the \textit{positive} class of the CR task \\
        \midrule
        The phone is very good looking with superb camera setup and very lightweight. \\
        Love this lens and it is affordable because it was used and works well with my camera. \\
        A great camera at a really great price This camera is easy to use with really good pictures. \\
        \midrule
        \bf Question types - Retrieved sentences for the \textit{location} class of the TREC task \\
        \midrule
        IN WHICH CITY IS THE HERMITAGE MUSEUM? \\
        Just where are the highlands of America? \\
        Lansing is the capital city of which state? \\
        \bottomrule
        \end{tabular}
        \smallskip
    }
    \caption{\small Examples of nearest neighbors using a sentence-level or label-level query for different domains.
    \label{tab:examples}}
    \end{table*}
           %\vspace{-0.4cm}

}



%%% Retrieval examples (shorter version)
\newcommand{\insertanalysis}{
    %{\tiny
    \begin{table*}[h!]
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{l}
        \toprule
        % \bf Examples of queries and nearest neighbors for various domains\\
        % \midrule
        \textbf{BioNLP query}: A single gene on chromosome 7 makes a protein called the cystic fibrosis transmembrane conductance regulator (CFTR).	 \\
        \textbf{Nearest neighbor}: Cystic Fibrosis A mutation in the gene cystic fibrosis transmembrane conductance regulator (CFTR) in chromosome 7. \\
        \midrule
        \textbf{Financial Query}: Google has entered into an agreement to buy Nest Labs for \$3.2 billion. \\
        \textbf{Nearest neighbor}: In January Google (NASDAQ:GOOG) reached an agreement to buy Nest Labs for \$3.2 billion in cash.\\
        \midrule
        \textbf{Hate-speech Query}: \textit{Average sentence embeddings of the "hateful" class of IMP} \\
        \textbf{Nearest neighbor}: fuzzy you are such a d* f* piece of s* just s* your g* d* mouth. -- All you n* and s* are fucking ret*\\
        \midrule
        \textbf{Movie review Query}: \textit{Average sentence embeddings of the "bad movie" class of SST-5} \\
        \textbf{Nearest neighbor}: This movie was terribly boring, but so forgettable as well that it didn't stand out for how awful it was.. \\
        \midrule
        \textbf{Product review Query}: \textit{Average sentence embeddings of the "positive" class of CR} \\
        \textbf{Nearest neighbor}: The phone is very good looking with superb camera setup and very lightweight. \\
        \midrule
        \textbf{Question type Query}: \textit{Average sentence embeddings of the "location" class of TREC} \\
        \textbf{Nearest neighbor}: Lansing is the capital city of which state? \\
        \bottomrule
        \end{tabular}
        \smallskip
    }
    \caption{\small Examples of nearest neighbors using a per-sentence or label-average query from different domains.
    \label{tab:analysis}}
    \end{table*}
           %\vspace{-0.4cm}

    %}
}


% STS results of SentAugment Sentence Embeddings (SASE)
\newcommand{\insertsts}{
    \begin{table}[h!]
        \begin{center}
            % \scriptsize
            \resizebox{1\linewidth}{!}{
            \begin{tabular}[b]{l|ccccc|c|c}
            \toprule
                \multirow{2}{*}{{Model}} & \multicolumn{6}{c|}{Semantic Textual Similarity (STS)} &  \\
                 & 2012 & 2013 & 2014 & 2015 & 2016 & Avg & STS-B \\
                %\midrule
                \midrule
                BERT (Mean) & 48.8 & 46.5 & 54.0 & 59.2 & 63.4 & 54.4 & - \\
                InferSent & 61.1 & 51.4 & 68.1 & 70.9 & 70.7 & 64.4 & 70.6  \\
                GenSen & 60.7 & 50.8 & 64.1 & 73.3 & 66.0 & 63.0 & -  \\
                USE & 61.4 & 59.0 & 70.6 & 74.3 & 73.9 & 67.8 & -  \\
                Sentence-BERT & 66.9 & 63.2 & 74.2 & 77.3 & 72.8 & 70.9 & -  \\
                uSIF- & 68.3 & {\bf 66.1} & {\bf 78.4} & 79.0 & - & - & 79.5  \\
                Word, trigram & 67.8 & 62.7 & 77.4 & 80.3 & 78.1 & 73.3 & 79.9  \\
                BGT & 68.9 & 62.2 & 75.9 & 79.4 & {\bf 79.3} & 73.1 & -  \\
                \midrule
                SASE (ours) & {\bf 69.7} & 62.9 & 77.3 & {\bf 79.8} & 78.1 & {\bf 73.5} & {\bf 80.8}  \\
                \bottomrule
            \end{tabular}
            }
            \caption{Results of our sentence encoder (SASE) on STS benchmarks from 2012 to 2016 and on the test sets of the STS-Benchmark dataset, compared to previously published results. We report Pearson’s r $\times$ 100. \label{tab:sts}}
        \end{center}
       \vspace{-0.4cm}
    \end{table}
}
